Adaptive Edge Offloading for Image Classification Under Rate Limit

This paper considers a setting where embedded devices are used to acquire and classify images. Because of limited computing capacity, embedded devices rely on a parsimonious classification model with uneven accuracy. When local classification is deemed inaccurate, devices can decide to offload the image to an edge server with a more accurate but resource-intensive model. Resource constraints, e.g., network bandwidth, however, require regulating such transmissions to avoid congestion and high latency. The paper investigates this offloading problem when transmissions regulation is through a token bucket, a mechanism commonly used for such purposes. The goal is to devise a lightweight, online offloading policy that optimizes an application-specific metric (e.g., classification accuracy) under the constraints of the token bucket. The paper develops a policy based on a Deep Q-Network (DQN), and demonstrates both its efficacy and the feasibility of its deployment on embedded devices. Of note is the fact that the policy can handle complex input patterns, including correlation in image arrivals and classification accuracy. The evaluation is carried out by performing image classification over a local testbed using synthetic traces generated from the ImageNet image classification benchmark. Implementation of this work is available at https://github.com/qiujiaming315/edgeml-dqn.

==> related_work_old.tex <==
\section{Related Work}

To address latency requirement and bandwidth constraints in edge computing settings that involve deep learning models, three general approaches have been explored to reduce the amount of data offloaded from devices to servers.

\begin{enumerate}[nosep, leftmargin=0pt, labelwidth=-15pt, labelsep=6pt, itemindent=0pt]

\item The \textit{model partitioning} approach targets Convolutional Neural Network (CNN) models and divides them between the device and the server~\cite{10.1145/3037697.3037698}. The device executes the first part of the model to generate intermediate results of smaller sizes than the original inputs, and offloads them to the server that completes the rest of model. The partitioning of the model depends on the specific structure of the CNN, which leaves no flexibility in enforcing different offloading rate limits. 

\item The second approach reduces the size of the offloaded data by \textit{adapting} the inputs to the model. A variety of techniques have been exploited to reduce the sizes of the inputs, including compression based on regions of interest (RoI)~\cite{ren2018distributed,liu2019edge}, adaptation of video frame size and rate \cite{liu2018dare}, deep compressive sensing \cite{yao2020deep}, and face cropping and contrast enhancement for emotion recognition \cite{muhammad2021emotion}.

\item The third approach employs a \textit{cascade} of models with increasing complexity and accuracy. The device runs a weak model and, as in our setting, offloads the input to the strong model on the server only if the weak model is not sufficiently confident of its output~\cite{DBLP:journals/corr/WangLCTG17,teerapittayanon2017distributed,liu2019edge}. Similar approaches have been used by video applications to adapt to network conditions~\cite{ananthanarayanan2019video,ran2018deepdecision}, where offloading and compression decisions depend on network connectivity.
\end{enumerate}

While the above approaches share the goal of reducing offloaded data, none seek to enforce explicit \textit{rate limits} as imposed by token buckets.  In contrast, our focus is on optimizing offloading decisions subject to token bucket constraints. In this work, we adopt the cascade of models framework while imposing rate constraints on the offloading decisions. While our focus is on cascade of models framework, we note that the framework also allows for input adaptation approaches that compress inputs the weak model decides to offload.  Such approaches are complementary to our solution and could readily be combined with it. We also note that our work is tailored to \textit{image} inputs (e.g., from image sensors) rather than video. As a result, we cannot take advantage of adaptation techniques specific to video streams such as those based on motion vectors and frame rates.  

The problem of optimizing offload decisions under token bucket constraint was introduced in~\cite{chakrabarti2020real} based on the cascade of models framework. This work is closest to ours and formulated the offloading decision problem as a Markov Decision Process (MDP) under the assumption of periodic and i.i.d.~inputs to the classifier. As alluded to in Section~\ref{sec:intro}, while those assumptions may be applicable in some limited settings, they are overly restrictive and unlikely to hold in many real-world applications.  Devising policies capable of handling complex (and arbitrary) image sequences is the focus and main contribution of this paper.

==> revision.tex <==
\section*{Revision Letter}

%This revision letter outlines the revisions we make to the paper for the second round of blind reviewing.  We first describe the main changes in this paper in detail and then respond to the questions or suggestions of each reviewer.  This letter describes how the reviewers' comments were addressed and responds to individual questions. 
Revisions are in \add{red} in the paper, with the comment(s) they seek to address listed in the margin. Editorial deletions to keep the paper to 12~pages are not shown.
%are not identified to reflect the paper's final form, but are mentioned as they arise.

\subsection{Changes}

%\add{
\begin{enumerate}[nosep]
\item We revised the abstract to highlight that our  offloading policy handles dependencies across inputs, and replaced ``inputs'' with ``images'' to make this focus explicit.
\item In response to comments M-2 and C-3, a few possible sample applications for the work were added in Section~\ref{sec:intro}.
\item In Section~\ref{sec:background}, the figure (former Fig.~3) and discussion illustrating different image arrival patterns were removed to keep the paper within 12 pages.
\item Section~\ref{sec:computation_offloading} was added to contrast our work against recent works on edge offloading in response to comments M-0, M-1, C-0, and C-1.
\item Section~\ref{sec:policy}'s heading was changed as it may have contributed confusion between offloading metric and reward.
\item In response to comments M-3, A-3, and B-1, the preamble of Section~\ref{sec:solution} was expanded to clarify the relation between offloading metric and reward and summarize the image processing pipeline.
\item An explanation of our choice of the DQN state space was added to Section~\ref{sec:dqn_setup} to address comments M-3, A-0, A-1, and B-1. We also included a brief discussion of our reasons for selecting DQN and our choice of network architecture
%explaining our choice of the RL algorithm and the DQN architecture
in response to comments M-2, A-4, and B-0.
\item As per comment A-6, we emphasized the testbed implementation in the preamble of Section~\ref{sec:evaluation}.
\item To address comment C-6, Section~\ref{sec:cost} now includes  information on the Raspberry Pi~4 and its configuration.  
\item Section~\ref{sec:dqn_param} now covers the impact of model architecture and parameters to address comments M-2 and B-0.
\end{enumerate}
%}
\subsection{Responses to Comments}
Responses to the meta review are numbered as M-$i$, with those for individual reviewers using A-$i$, B-$i$, C-$i$, respectively. % Each response starts with a quote of the corresponding comment.

\vspace{6pt}
\subsubsection{\bf Responses to Meta Review}\hfill

\review{M-0}{The paper can benefit from a more complete review of the existing work on offloading \ldots % For closely related work, the authors should make clear how the proposed approach is different or better.
}

We thank reviewer 3 for pointing out several relevant recent works on offloading algorithms that we had indeed missed in our review of prior work. Section~\ref{sec:computation_offloading} now discusses those works and contrasts them with our approach, including why extending them to our problem is not immediate.

\review{M-1}{The experiments may compare with possibly more recent work that represents the state-of-the-art.
}

%\add{
We reviewed works from the survey cited by reviewer~3, but while their motivations and settings intersect those of the paper, there are many differences so that their results cannot be directly applied.   Section~\ref{sec:computation_offloading} reviews these differences.
%}

\review{M-2}{The experiment may add an evaluation on the impact of the number of \ldots % units in the perceptrons or the number of layers. 
It may also consider a real setting \ldots % with more realistic image streams.
}

We apologize for the omission and are now reporting the results of a set of experiments consisting of a full grid search of the model's parameters 
%impact of the model architecture on performance 
in Section \ref{sec:dqn_param}.

Demonstrating our system with a realistic image stream would indeed be more convincing.  Unfortunately, we could not identify a relevant dataset.
%an existing dataset representative of the environment we target.
Video analytics datasets are the closest fit, but are not really suitable as: (1) They usually target object detection or image segmentation rather than image classification; (2) Inter-arrival times are hardly variable; (3) Consecutive video frames are correlated, but this is because of similarity in content rather than in classification confidence. This latter aspect could be addressed by down-sampling frames, but this significantly reduces the datasets which results in insufficient training data.  Alternatively, we could have generated our own dataset, but there was not enough time to do so. Instead, to better illustrate the practical relevance of the work, we opted to mention in Section~\ref{sec:intro} a few real-world applications to which it could apply. 
%\rg{I don't have a good alternative, but I found this relatively weak.}

\review{M-3}{The paper may better justify the assumption that the result from the strong classifier is known at the next time.}

Our solution does not require knowing the strong classifier's result at the next time for its offloading decision. A clarification to that effect was added in Sections \ref{sec:solution} and \ref{sec:dqn_setup}.

\vspace{6pt}
\subsubsection{\bf Response to Reviewers}\hfill

\review{A-0}{The state-space used in the system could be described a little bit more.}

A more detailed description is now in Sections~\ref{sec:solution} and~\ref{sec:dqn_setup}, which hopefully clarifies the state space definition and choice.

\review{A-1}{The choice of not using raw images for the DQN inputs should be discussed.}

A discussion of this choice was added in Section~\ref{sec:dqn_setup}.

\review{A-2}{The modelization choice consisting in using a finite history window could be challenged \ldots}
%by the use of a recurrent neural network architecture in the Q-network.}

An RNN model has indeed advantages in handling sequential data, which could yield a better offloading policy.  However, the computational footprint of RNNs is very challenging for the kind of embedded devices we target. Preserving computational simplicity was our focus and the main reason for limiting ourselves to a simple MLP architecture.
%since one of our goal is to develop an efficient solution for making offloading decisions at local devices, we choose to stick with the simple MLP architecture in this paper and consider RNN in our future work.  
We plan to explore the possibility of fitting an RNN-based solution on embedded devices as part of future work, and a brief discussion to that effect was added to Section~\ref{sec:dqn_setup}.

\review{A-3}{It is not clear to me why it is necessary to estimate the offloading reward \ldots }%.  Since all classifiers are already trained, why could we not just pre-compute offline the offloading metrics using both classifier's predictions on the data that will be used during training?}

%Note that offloading reward and offloading metric are distinct quantities.  
The offloading \emph{reward} for an image $x$ is either -1, 0, or 1 depending on the respective classification outcomes of the two classifiers. %(\ie either right or wrong). 
In contrast, 
%as discussed in Section~\ref{sec:metric}, 
the offloading \emph{metric} $m(x)$ is a real value in $[-1, 1]$, which is an estimate of the expected value of this reward using only the weak classifier (the entropy $h(\mathcal{W}(x))$ of its output).  As illustrated in \fig{fig:offloading_metric}, this estimate is pre-computed during training as the reviewer suggests.  Details were added in Section~\ref{sec:solution} to hopefully clarify those concepts.

\review{A-4}{\ldots 
%DQN is an efficient and straightforward algorithm but 
some more recent algorithms, such as PPO or Rainbow, generally outperform DQN \ldots } %. Authors may consider comparing their method using the same setting but a different RL algorithm leading to some possible performance improvements.}

Thank you for pointing to these recent RL algorithms, which could potentially offer some performance improvements.  Because our state space is relatively simple compared to high-dimensional inputs such as raw images, we expect the benefits of more sophisticated algorithms over DQN to be limited.  However, investigating whether this is the case is of interest and something we plan to do in future work.  We have added a statement to that effect at the end of Section~\ref{sec:dqn_setup}. 
%\rg{I will note that this is a rather weak response.  A stronger one would have been to say that we tried one of those algorithms and did not find much improvement.  But I understand that we may not have the time for that.}

\review{A-5}{%The method already outperforms the MDP and baselines methods. This demonstrates the 
\ldots interest in using a policy learned by an RL agent to optimize  distributed image classification systems.}

Thank you for the suggestion.  Extending the work to a distributed setting is indeed a natural nest step, one we are targeting as a next phase for the work.  
%Using the DQN-based offloading policy in a distributed edge computing system is one of the most interesting extension to this work and we will investigate that in our future work.  
The biggest challenge is one present in multi-agent reinforcement learning systems, where devices have to infer the states of others from the edge server's responses. Devising effective and parsimonious solutions for such inference is an intriguing question.
%that the problem in this setting requires some knowledge of multi-agent reinforcement learning (MARL), where each device needs to infer the states of the other devices using the response it receives from the edge server.

\review{A-6}{
%Despite this, the experimental part is interesting, and
\ldots it should be emphasized that the experiments were performed on a real physical system \ldots }
%instead of on a simulator (and with an actual test set which is unfortunately not always the case in RL).}

Thank you and we have highlighted this in Section~\ref{sec:evaluation}.

%\subsubsection{Response to Review 2}\hfill
%\smallskip
\noindent
\hrulefill

\review{B-0}{The architecture of the DQN is arbitrary \ldots 
%and there is no discussion of the reasons behind such choice or 
the impact of the hyper-parameters values on the efficacy of the DQN.}

%\rg{We still need to justify the choice of architecture. This is different from the grid search.}
Thank you for pointing out the need for those discussions.  The reasons for our choice of a relatively simple architecture have been 
%\add{
added to Section \ref{sec:dqn_setup}.
%}
Conversely, to understand the impact of the model's hyper-parameters (number of layers and number of units per layer) we carried out a grid search that revealed a relative insensitivity to their values.  We have added a discussion of both aspects in Section~\ref{sec:dqn_param}.

\review{B-1}{The proposed solution requires to know the inference result for the previous input sample \ldots } %before to be able to treat the next sample. This does not allow for execution pipelining, thus decreasing throughput.}

We apologize for not making this clearer, but the  proposed solution does not require the inference result of the strong classifier to make the next offloading decision.  Towards eliminating the potential for confusion, we have added an explicit discussion to that effect in both Sections~\ref{sec:solution} and~\ref{sec:dqn_setup}.

\review{B-2}{The presentation of the architecture of the DQN is ambiguous and thus confusing.}

We have sought to address this concern by clarifying the architecture of the system and adding details in Section~\ref{sec:dqn_setup}.
%Thanks for the detailed comment.  We have rephrased that sentence in Section \ref{sec:dqn_setup} according to your suggestion.

%\subsubsection{Response to Review 3}\hfill
%\smallskip
\noindent
\hrulefill

\review{C-0, C-1}{The literature survey may not be complete on offloading algorithms.  The experiments may compare with possibly more recent work that represents the state-of-the-art.}
% \review{C-0}{The literature survey may not be complete on offloading algorithms.}

% Please see our response to M-0.
%Thanks for reminding us of this omission and the surveys you pointed to are really helpful resources.  We have added a new sub-section \ref{sec:computation_offloading} in related work to review these algorithms, discuss how they are related to our work, and explain why these works are different from ours and why they cannot be trivially extended to our targeted problem.

% \review{C-1}{The experiments may compare with possibly more recent work that represents the state-of-the-art.}

%\add{
Please see our responses to M-0 and M-1, respectively.
%}

\review{C-2}{The paper is specific to applications that classify inputs. I think this should be reflected in the title.}

This is absolutely correct, and we would be happy to update the title accordingly if allowed.
%Thanks for your suggestion and we think it is a good idea to highlight image classification as our target application in the title.  \JQadd{Either change the title, or explain why we cannot do so and how we revise the abstract according to this suggestion}.

\review{C-3}{%The experimental evaluation is based on synthetic traces for image classification.  
\ldots It can be better to have a real setting such that the input process reflects a more realistic image stream.}

Please see our response to the second part of M-2.
%Unfortunately, we could not locate a dataset derived from a real-world application and generating one was not feasible within the available time. However, we added a discussion of potential applications in Section \ref{sec:intro}.  More details are in M-2.

\review{C-4}{%Also, do we consider battery-powered embedded devices?  
\ldots If so, a measurement on the energy consumption will be useful as well.}

As discussed in Section~\ref{sec:computation_offloading}, several works develop offloading algorithms under energy constraints, which is not an aspect we consider. The optimization framework it gives rise to differs significantly from that of the token bucket constraints we face.  However, we believe that it may be possible to extend our framework to incorporate this additional constraint, and plan to investigate such an extension as part of future work.
%in related work how our work is related to other offloading algorithms that considers energy consumption.  We will consider energy consumption as an extension in our future work.

\review{C-5}{Is it also possible to plot the most accurate offloading results? \ldots}% In this way, we can know how far away the DQN approach is from the optimal solution.}

The ``lower bound'' policy that offloads the fraction of images with the highest possible reward provides a possible reference point, but one that is infeasible since it ignores the bucket depth constraint of the token bucket. Unfortunately, characterizing the ``optimal'' policy appears intractable, so that we are unable to better assess the optimality gap of the DQN policy beyond comparing it to the ``lower bound.''.
%Unfortunately, the ``optimal'' offloading policy depends both on the correlation pattern of the image sequence, the token bucket constraints, and the approach to evaluate the offloading reward of each image using only the weak classifier output, which is very complicated (if not impossible) to analyze exactly even offline.  Therefore, we cannot provide anything better than the lower bound (which is an infeasible policy in our problem setting since it assumes infinite bucket depth) as an indicator of the room for improvement.

\review{C-6}{What is the specification of the embedded device Raspberry Pi 4B? How much does it cost?}

Those details have now been added to Section~\ref{sec:testbed}.
%Thank you for highlighting the importance of mentioning the hardware specification.  It is now added to Section \ref{sec:testbed}.

